First direct constraints on Fierz interference in free neutron $\beta$ decay

Precision measurements of free neutron $\beta$-decay have been used to precisely constrain our understanding of the weak interaction. However the neutron Fierz interference term $b_n$, which is particularly sensitive to Beyond-Standard-Model tensor currents at the TeV scale, has thus far eluded measurement. Here we report the first direct constraints on this term, finding $b_n = 0.067 \pm 0.005_{\text{stat}} {}^{+0.090}_{- 0.061}{}_{\text{sys}}$, consistent with the Standard Model. The uncertainty is dominated by absolute energy reconstruction and the linearity of the beta spectrometer energy response.

==> UCNA_2010_Authors.tex <==
\author{K.~P.~Hickerson}		\affiliation{Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, California 91125, USA} %\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 

\author{Y.~Bagdasarova}		\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} \affiliation{Department of Physics, University of Washington, Seattle, Washington 98195, USA} 
\author{D.~B.~Berguno}		\affiliation{Department of Physics, Virginia Tech, Blacksburg, Virginia 24061, USA} 
\author{L.~J.~Broussard}		\affiliation{Department of Physics, Duke University, Durham, North Carolina 27708, USA} 
\author{M.~Brown}			\affiliation{Department of Physics and Astronomy, University of Kentucky, Lexington, Kentucky 40506, USA} 
\author{R.~Carr}			\affiliation{Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, California 91125, USA} 
\author{S.~Currie}			\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 
\author{X.~Ding}			\affiliation{Department of Physics, Virginia Tech, Blacksburg, Virginia 24061, USA} 
\author{B.~W.~Filippone}		\affiliation{Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, California 91125, USA} 
\author{A.~Garc\'ia}			\affiliation{Department of Physics, University of Washington, Seattle, Washington 98195, USA} 
\author{P.~Geltenbort}		\affiliation{Institut Laue-Langevin, 38042 Grenoble Cedex 9, France} 
\author{J.~Hoagland}		\affiliation{Department of Physics, North Carolina State University, Raleigh, North Carolina 27695, USA} 
%\author{G.~E.~Hogan}		\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA}
\author{A.~T.~Holley}		\affiliation{Department of Physics, North Carolina State University, Raleigh, North Carolina 27695, USA} \affiliation{Department of Physics, Indiana University, Bloomington, Indiana 47408, USA} 
\author{R.~Hong}			\affiliation{Department of Physics, University of Washington, Seattle, Washington 98195, USA} 
\author{T.~M.~Ito}			\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 
\author{A.~Knecht}			\affiliation{Department of Physics, University of Washington, Seattle, Washington 98195, USA} 
\author{C.-Y.~Liu}			\affiliation{Department of Physics, Indiana University, Bloomington, Indiana 47408, USA} 
\author{J.~L.~Liu}			\affiliation{Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, California 91125, USA}  \affiliation{Department of Physics, Shanghai Jiao Tong University, Shanghai 200240, China}
\author{M.~Makela}			\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 
\author{R.~R.~Mammei}		\affiliation{Department of Physics, Virginia Tech, Blacksburg, Virginia 24061, USA} 
\author{J.~W.~Martin}		\affiliation{Department of Physics, University of Winnipeg, Winnipeg, MB R3B 2E9, Canada} 
\author{D.~Melconian}		\affiliation{Cyclotron Institute, Texas AM University, College Station, Texas 77843, USA} 
\author{M.~P.~Mendenhall}	\affiliation{Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, California 91125, USA} 
\author{S.~D.~Moore}		\affiliation{Department of Physics, North Carolina State University, Raleigh, North Carolina 27695, USA} 
\author{C.~L.~Morris}		\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 
\author{R.~W.~Pattie,~Jr.}		
	%\affiliation{Department of Physics, North Carolina State University, Raleigh, North Carolina 27695, USA} 
	\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 
\author{A.~P\'erez Galv\'an}	\thanks{Currently at Physics Division, Argonne National Laboratory, Argonne, IL 60439, USA} \affiliation{Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, California 91125, USA}  
\author{R.~Picker}			\affiliation{Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, California 91125, USA} 
\author{M.~L.~Pitt}			\affiliation{Department of Physics, Virginia Tech, Blacksburg, Virginia 24061, USA} 
\author{B.~Plaster}			\affiliation{Department of Physics and Astronomy, University of Kentucky, Lexington, Kentucky 40506, USA} 
\author{J.~C.~Ramsey}		\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 
\author{R.~Rios}			\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} \affiliation{Department of Physics, Idaho State University, Pocatello, Idaho 83209, USA} 
\author{A.~Saunders}		\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 
\author{S.~J.~Seestrom}		\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA}
\author{E.~I.~Sharapov}		\affiliation{Joint Institute for Nuclear Research, 141980, Dubna, Russia} 
\author{W.~E.~Sondheim}	\affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 
\author{X.~Sun}			\affiliation{Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, California 91125, USA} 
\author{E.~Tatar}			\affiliation{Department of Physics, Idaho State University, Pocatello, Idaho 83209, USA} 
\author{R.~B.~Vogelaar}		\affiliation{Department of Physics, Virginia Tech, Blacksburg, Virginia 24061, USA} 
\author{B.~VornDick}		\affiliation{Department of Physics, North Carolina State University, Raleigh, North Carolina 27695, USA} 
\author{C.~Wrede}			\thanks{Currently at Department of Physics and Astronomy and National Superconducting Cyclotron Laboratory, Michigan State University, East Lansing, Michigan 48824, USA} \affiliation{Department of Physics, University of Washington, Seattle, Washington 98195, USA}  
\author{A.~R.~Young}		\affiliation{Department of Physics, North Carolina State University, Raleigh, North Carolina 27695, USA} 
\author{B.~A.~Zeck}			\affiliation{Department of Physics, North Carolina State University, Raleigh, North Carolina 27695, USA} \affiliation{Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA} 

\collaboration{UCNA Collaboration}
